Routes Towards Optical Quantum Technology --- New Architectures and Applications

This thesis is based upon the work I have done during my PhD candidature at Macquarie University. In this work we develop quantum technologies that are directed towards realising a quantum computer. Specifically, we have made many theoretical advancements in a type of quantum information processing protocol called BosonSampling. This device efficiently simulates the interaction of quantum particles called bosons, which no classical computer can efficiently simulate. In this thesis we explore quantum random walks, which are the basis of how the bosons in BosonSampling interfere with each other. We explore implementing BosonSampling using the most readily available photon source technology. We invented a completely new architecture which can implement BosonSampling in time rather than space and has since been used to make the worlds largest BosonSampling experiment ever performed. We look at variations to the traditional BosonSampling architecture by considering other quantum states of light. We show a worlds first application inspired by BosonSampling in quantum metrology where measurements may be made more accurately than with any classical method. Lastly, dealing with BosonSampling, we look at reformulating the formalism of BosonSampling using a quantum optics approach. In addition, but not related to BosonSampling, we show a protocol for efficiently generating large-photon Fock states, which are a type of quantum state of light, that are useful for quantum computation. Also, we show a method for generating a specific quantum state of light that is useful for quantum error correction --- an essential component of realising a quantum computer --- by coupling together light and atoms.

==> Sections/listofsymbols.tex <==
\chapter{List of Symbols}

% please change this list to suit your thesis

\begin{list}{}{%
\setlength{\labelwidth}{24mm}
\setlength{\leftmargin}{35mm}}
\item[$a$, $b$, $c$, $d$\dotfill] annihilation operators
\item[$a^\dagger$, $b^\dagger$, $c^\dagger$, $d^\dagger$\dotfill] creation
operators
\end{list}

